Bounded Model Checking for Probabilistic Programs

In this paper we investigate the applicability of standard model checking approaches to verifying properties in probabilistic programming. As the operational model for a standard probabilistic program is a potentially infinite parametric Markov decision process, no direct adaption of existing techniques is possible. Therefore, we propose an on-the-fly approach where the operational model is successively created and verified via a step-wise execution of the program. This approach enables to take key features of many probabilistic programs into account: nondeterminism and conditioning. We discuss the restrictions and demonstrate the scalability on several benchmarks.

==> Makefile <==
.PHONY: default clean distclean


default: main.pdf


main.pdf: *.tex ../../bibliography.bib
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main


clean:
	rm -f *.aux *.log *.bbl *.blg *~ main.pdf *.out *.synctex.gz

distclean: clean
	rm -f main.pdf


==> pics/operational_example.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,node distance=2.7cm,semithick,minimum size=1cm]
\tikzstyle{every state}=[draw=none]
  \draw[white, use as bounding box] (-6.6,-6.3) rectangle (3.4,0.3);
   \node [state, initial where=above, initial text=] (init) at (0,0) {$\langle P,\,\sigma_I \rangle$};  
    \node [] (s1) [on grid, below=1.5 cm of init, xshift=-2.2cm] {$\langle P_1;\,P_3,\,\sigma_I\rangle$};   
%    \node [] (s2) [on grid, below=1.5 cm of init, xshift=2.2cm] {$\langle P_2;\,P_3,\,\sigma_I\rangle$};   
        \node [] (s11) [on grid, below=1.5 cm of init, xshift=2.2cm] {$\langle P_2;\,P_3,\,\sigma_I\rangle$};   
        \node [] (s12) [on grid, left=2 cm of s1, xshift=-1.2cm] {$\langle P_4;\,P_3,\,\sigma_I\rangle$};   
%        \node [] (s21) [on grid, below=1.5 cm of s2] {$\langle\term;\,P_3,\,\sigma_I\subst x 2\rangle$};   
        \node [] (s111) [on grid, below=1.5 cm of s11] {$\langle\term;\,P_3,\,\sigma_I\subst x 2\rangle$};   
        \node [] (s121) [on grid, below=1.5 cm of s12] {$\langle\term;\,P_3,\,\sigma_I\subst x 5\rangle$};   
%        \node [] (s211) [on grid, below=1.5 cm of s21] {$\langle P_3,\,\sigma_I\subst x 2\rangle$};   
         \node [] (s1111) [on grid, below=1.5 cm of s111] {$\langle\,P_3,\,\sigma_I\subst x 2\rangle$};   
         \node [] (s1211) [on grid, right=3.3 cm of s121] {$\langle P_3,\,\sigma_I\subst x 5\rangle$};   
         \node [label={[yshift=0.0cm, gray] 180:$5$}] (s12111) [on grid, below=1.5 cm of s1211] {$\langle\term,\,\sigma_I\subst x 5\rangle$};   
 \node [] (undesired) [on grid, below=1.5 cm of s1111, xshift=-.5cm] {$\undesired$};  
  \node [] (sink) [on grid, below=1.5 cm of s12111, xshift=1.5cm] {$\sink$};  

\path
      (init) edge [] node [left, near start] {\scriptsize{$q$}} (s1)
      (init) edge [] node [right, near start] {\scriptsize{$1-q$}} (s11)
      (s1) edge [] node [below=-0.3cm] {\scriptsize{$\mathit{left}$}} (s12)
      (s1) edge [] node [below=-0.3cm] {\scriptsize{$\mathit{right}$}} (s11)
%      (s2) edge [] (s21)
      (s12) edge [] (s121)
      (s11) edge [] (s111)
      (s111) edge [] (s1111)
      (s121) edge [] (s1211)
%      (s21) edge [] (s211)
      (s1111) edge [] (undesired)
      (s1211) edge [] (s12111)
%      (s211) edge [] (undesired)
      (undesired) edge [] (sink)
      (s12111) edge [] (sink)
      (sink) edge [loop above] (sink)
;
\end{tikzpicture}

